Semantic Parsing in Limited Resource Conditions

This thesis explores challenges in semantic parsing, specifically focusing on scenarios with limited data and computational resources. It offers solutions using techniques like automatic data curation, knowledge transfer, active learning, and continual learning. For tasks with no parallel training data, the thesis proposes generating synthetic training examples from structured database schemas. When there is abundant data in a source domain but limited parallel data in a target domain, knowledge from the source is leveraged to improve parsing in the target domain. For multilingual situations with limited data in the target languages, the thesis introduces a method to adapt parsers using a limited human translation budget. Active learning is applied to select source-language samples for manual translation, maximizing parser performance in the target language. In addition, an alternative method is also proposed to utilize machine translation services, supplemented by human-translated data, to train a more effective parser. When computational resources are limited, a continual learning approach is introduced to minimize training time and computational memory. This maintains the parser's efficiency in previously learned tasks while adapting it to new tasks, mitigating the problem of catastrophic forgetting. Overall, the thesis provides a comprehensive set of methods to improve semantic parsing in resource-constrained conditions.

==> Chapters/Chapter1.tex <==
\chapter{Introduction}

\section{Writing a thesis}
Writing a thesis is a lengthy process, often requiring multiple redrafts and revisions.

Drafts should be provided and reviewed on a regular basis to keep up momentum as the submission deadline approaches. Please ensure that all required milestones and program requirements (e.g. professional development hours) have been completed before progressing with your submission.

The information below has been provided to you to make your experience as easy as possible. You may also like to refer to the Graduate Research Thesis Examination Procedures for further insight into the thesis examination process.

\subsection{what format the thesis will be presented}
The first thing to consider is in what format the thesis will be presented.
We recommend students and main supervisors discuss this as early as possible, and jointly agree on the most appropriate option:

Traditional thesis: A similar format to research reports and papers where the research question is proposed, methodology is described and the results are discussed and conclusions established.

Thesis including published works: Overall format is the same as a traditional thesis but particular chapters will include any submitted publications. Some Faculties have their own criteria for what can be included in this format.

All theses must use the approved thesis preliminary pages which includes compulsory information such as copyright and authorship declarations. If these pages are not presented correctly, the thesis will not be dispatched to the examiners and the relevant sections will need to be amended.

\subsection{examiners}
At Monash each graduate research student has a supervisory team. Of this group, the main supervisor is responsible for approaching potential examiners for their students' thesis. Initial discussions normally take place at the student’s final milestone review and it is recommended that examiners are approached at least 4-6 weeks before expected submission.

An email template is available for use when inviting potential examiners to examine a thesis.

For students enrolled in a Live Music or Theatre Performance degree, the main supervisor will also need to complete a Nomination of Examiners form. This form will require the approval of the Program Director (or delegate) and the Monash Graduate Research Office prior to the live performance. For further information please contact the Faculty of Arts.

In addition, when considering appropriate examiners, please note that if an examiner is subject to Sanctions laws, we are unable to provide payment for their thesis examination.

\subsection{conflict of interest}
There are a range of circumstances that could result in a conflict of interest, potentially restricting the objectivity of the examiners.

Some examples of what we consider conflicts of interest are:

Involvement in the student's research, including supervision of the candidate in field or laboratory work or elsewhere during candidature.
Previous work in the same department within an institution as the candidate.
A previous appointment as an academic staff member at Monash University, including an adjunct academic appointment, during the student’s period of candidature.
Holding the position of emeritus or adjunct professor at Monash.
Substantial contact with the candidate in any other circumstance which might jeopardise the independence of the examination.
Being a close associate (spouse/partner, other relative, friend or business partner) of either the candidate or the supervisor of the candidate.
There is a more comprehensive list of grounds for conflicts of interest which you may wish to review.


\section{Thesis including Published Works}
All doctoral and research master's students are permitted to submit a thesis including published works, in accordance with section 1.9 of the Graduate Research Thesis Examination Procedures. The thesis including published works is not a different degree; rather, it is a thesis format that includes papers that have been submitted, or accepted, for publication, during the course of the student's enrolment in the relevant graduate research degree at Monash.

The thesis must reflect a sustained and cohesive theme, and framing or substantial linking text is normally required in introducing the research and linking the chapter/papers/manuscripts. The papers do not have to be rewritten for the thesis. For guidance, refer to Text Framing the Publications (as below).

Whether the papers are required to have been published, accepted for publication, or only submitted for publication varies across faculties (see Faculty Requirements below). We advise you to consult good examples of theses including published works in your discipline. Your academic unit or school should have copies of all doctoral and research master's theses available for consultation. Workshops on the thesis including published works are also run through the Skills Essentials series, if you require more information.


\section{The maximum word length}
For references see \href{http://www.monash.edu/__data/assets/pdf_file/0011/911882/Graduate-Research-Thesis-Examination-Procedures.pdf}{Graduate Research Thesis Examination Procedures} 

PhD: 80,000 words,  100,000 words for students enrolled prior to 1 January 2015

MPhil: 35,000 words, 50,000 words for students enrolled prior to 1 January 2015.

\section{Using Figures and Tables, and other commands}

We have defined several commands in thesis.cls file for easier usage:
\begin{verbatim}
\newcommand{\fref}[1]{Figure~\ref{#1}}
\newcommand{\tref}[1]{Table~\ref{#1}}
\newcommand{\eref}[1]{Equation~\ref{#1}}
\newcommand{\cref}[1]{Chapter~\ref{#1}}
\newcommand{\sref}[1]{Section~\ref{#1}}
\newcommand{\aref}[1]{Appendix~\ref{#1}}
\renewcommand{\topfraction}{0.85}
\renewcommand{\bottomfraction}{.85}
\renewcommand{\textfraction}{0.1}
\renewcommand{\dbltopfraction}{.85}
\renewcommand{\floatpagefraction}{0.75}
\renewcommand{\dblfloatpagefraction}{.75}
\end{verbatim}

You can use \textit{fref} and \textit{tref} to refer a figure and table, such as \fref{fig.demo1} and \tref{table.demo1}. Refer a citation like this \cite{Reference1}. You can cite multiple references once, like this \cite{Reference1,Reference2,Reference3}.



\begin{figure}
\centering
  \includegraphics[width=8cm,height=5cm]{Figures/crest.jpg}%
  \caption{My Picture Demo\label{fig.demo1}}
\end{figure}

\begin{table}[]
\caption{Table Demo.\label{table.demo1}}
\begin{tabular}{|c|c|c|}
\hline
Description & Images &  \\ \hline
Training & Taking 3 images of knowns + 1 image of known unknowns randomly & 2,900 \\ \hline
Gallery & Taking 3 images of knowns randomly & 1,830 \\ \hline
Probe C & C=S & 4,903 \\ \hline
Probe O1 & O1 & 6,264 \\ \hline
Probe O2 & O2 & 8,972 \\ \hline
Probe O3 & O3 & 10,333 \\ \hline
\end{tabular}
\end{table}

\section{A Section}

Quisque tristique urna in lorem laoreet at laoreet quam congue. Donec dolor turpis, blandit non imperdiet aliquet, blandit et felis. In lorem nisi, pretium sit amet vestibulum sed, tempus et sem. Proin non ante turpis. Nulla imperdiet fringilla convallis. Vivamus vel bibendum nisl. Pellentesque justo lectus, molestie vel luctus sed, lobortis in libero. Nulla facilisi. Aliquam erat volutpat. Suspendisse vitae nunc nunc. Sed aliquet est suscipit sapien rhoncus non adipiscing nibh consequat. Aliquam metus urna, faucibus eu vulputate non, luctus eu justo.

\subsection{A Subsection}

Donec urna leo, vulputate vitae porta eu, vehicula blandit libero. Phasellus eget massa et leo condimentum mollis. Nullam molestie, justo at pellentesque vulputate, sapien velit ornare diam, nec gravida lacus augue non diam. Integer mattis lacus id libero ultrices sit amet mollis neque molestie. Integer ut leo eget mi volutpat congue. Vivamus sodales, turpis id venenatis placerat, tellus purus adipiscing magna, eu aliquam nibh dolor id nibh. Pellentesque habitant morbi tristique senectus et netus et malesuada fames ac turpis egestas. Sed cursus convallis quam nec vehicula. Sed vulputate neque eget odio fringilla ac sodales urna feugiat.

\section{Another Section}

Phasellus nisi quam, volutpat non ullamcorper eget, congue fringilla leo. Cras et erat et nibh placerat commodo id ornare est. Nulla facilisi. Aenean pulvinar scelerisque eros eget interdum. Nunc pulvinar magna ut felis varius in hendrerit dolor accumsan. Nunc pellentesque magna quis magna bibendum non laoreet erat tincidunt. Nulla facilisi.

Duis eget massa sem, gravida interdum ipsum. Nulla nunc nisl, hendrerit sit amet commodo vel, varius id tellus. Lorem ipsum dolor sit amet, consectetur adipiscing elit. Nunc ac dolor est. Suspendisse ultrices tincidunt metus eget accumsan. Nullam facilisis, justo vitae convallis sollicitudin, eros augue malesuada metus, nec sagittis diam nibh ut sapien. Duis blandit lectus vitae lorem aliquam nec euismod nisi volutpat. Vestibulum ornare dictum tortor, at faucibus justo tempor non. Nulla facilisi. Cras non massa nunc, eget euismod purus. Nunc metus ipsum, euismod a consectetur vel, hendrerit nec nunc.

==> Preamble/Declaration_publications.tex <==
% https://www.monash.edu/graduate-research/examination/publication
% https://www.monash.edu/rlo/graduate-research-writing/write-the-thesis
% https://www.monash.edu/rlo/graduate-research-writing/write-the-thesis/writing-the-thesis-chapters/structuring-a-long-text
\Declarationpublication{
\addtocontents{toc}{}  % Add a gap in the Contents, for aesthetics

\emph{This declaration is to be included in a `thesis including published works'. You must provide details of all publications included in your thesis in the section below. If you have not completed a thesis including published works.}

\emph{Please ensure your thesis meets the \href{https://www.monash.edu/graduate- esearch/examination/publication}{thesis including published works requirements}. Some faculties vary requirements in terms of the number of papers required, status of papers
and other criteria. These faculty specific requirements can also be found at the above link.}

\emph{Please remove the above section and include a standard thesis declaration.}

I hereby declare that this thesis contains no material which has been accepted for the award of any other degree or diploma at any university or equivalent institution and that, to the best of my knowledge and belief, this thesis contains no material previously published or written by another person, except where due reference is made in the text of the
thesis.

This thesis includes (\emph{insert number)} original papers published in peer reviewed journals and (\emph{insert number)} submitted publications. The core theme of the thesis is (\emph{insert theme}). The ideas, development and writing up of all the papers in the thesis were the principal responsibility of myself, the student, working within the
(\emph{insert name of academic unit}) under the  supervision of (\emph{insert name of supervisor}).

(The inclusion of co-authors reflects the fact that the work came from active collaboration between researchers and acknowledges input into
team-based research.) \emph{Remove this paragraph for theses with sole-authored work}

In the case of \emph{(insert chapter numbers}) my  contribution to the work involved the following:

\emph{(If this is a laboratory-based discipline, a paragraph outlining the assistance given during the experiments, the nature of the experiments and an attribution to the contributors could follow.})

Here should be the table!

I have / have not renumbered sections of submitted or published papers
in order to generate a consistent presentation within the thesis.

Student name:

Student signature: Date:

I hereby certify that the above declaration correctly reflects the
nature and extent of the student's and co-authors' contributions to this
work. In instances where I am not the responsible author I have
consulted with the responsible author to agree on the respective
contributions of the authors.

\textbf{Main Supervisor name:}

\textbf{Main Supervisor signature:} \textbf{Date:}


}

==> Preamble/Preface.tex <==
% https://www.monash.edu/graduate-research/examination/publication
% https://www.monash.edu/rlo/graduate-research-writing/write-the-thesis
% https://www.monash.edu/rlo/graduate-research-writing/write-the-thesis/writing-the-thesis-chapters/structuring-a-long-text
\Preface{

\addtocontents{toc}{}  % Add a gap \vspace{1em} in the Contents, if for aesthetics

Where applicable, the following information must be included in a preface:
\begin{itemize}
\item[\tiny{$\blacksquare$}] a description of work towards the thesis that was carried out in collaboration with others, indicating the nature and proportion of the contribution of others and in general terms the portions of the work which the student claims as original;
\item[\tiny{$\blacksquare$}] a description of work towards the thesis that has been submitted for other qualifications;
\item[\tiny{$\blacksquare$}] a description of work towards the thesis that was carried out prior to enrolment in the degree;
\item[\tiny{$\blacksquare$}] whether any third-party editorial assistance was provided in preparation of
the thesis and whether the persons providing this assistance are knowledgeable in the academic discipline of the thesis;
\item[\tiny{$\blacksquare$}] the contributions of all persons involved in any multi-authored publications or
articles in preparation included in the thesis;
\item[\tiny{$\blacksquare$}] the publication status of all chapters presented in article format using the
descriptors below;
    \begin{itemize}
        \item Unpublished material not submitted for publication
        \item Submitted for publication to [publication name] on [date]
        \item In revision following peer review by [publication name]
        \item Accepted for publication by [publication name] on [date]
        \item Published by [publication name] on [date]
    \end{itemize}
\item[\tiny{$\blacksquare$}] an acknowledgement of all sources of funding, including grant identification
numbers where applicable and Australian Government Research Training Program Scholarships, including fee offset scholarships.
\end{itemize}

}

==> Tables/simple_complex.tex <==
\begin{table}[]
\begin{tabular}{l|cc}
\hline
\multirow{2}{*}{\textbf{Training   Data}} & \multicolumn{2}{l}{\textbf{Logic Form-Exact Matching}} \\ \cline{2-3} & Simple & complex   \\ \hline
Original training dataset & 42.18  &  30.36 \\
With Filtered BT (Spanish) & 42.18 & 28.57 \\
With Filtered BT (Chinese) & 44.13  & 29.46 \\
With Filtered BT (Telugu)  & 43.20 & 29.76 \\
With Filtered GPT-3 & 45.92  & 31.70 \\
With Filtered BART & 44.22 & 28.57 \\
With Filtered Quillbot & \textbf{50.00} & \textbf{42.86} \\
Full Filtered Data & 45.58 & 40.03 \\ \hline
\end{tabular}
% \vspace{0.2 cm}
\caption{question types analyses}
\label{tab:simple_complex}
\end{table}

==> Tables/tab-local_exp.tex <==
\begin{table}[ht] % title of Table
\centering % used for centering table
{\small
\begin{tabular}{l l} % centered columns (4 columns)
\hline\hline %inserts double horizontal lines
$\text{D}$ & Database about pets \\ % inserts table
%heading
\hline % inserts single horizontal line
$\text{Q}_1$ & What are the different pet types? \\
$\text{S}_1$ & 
SELECT DISTINCT pettype FROM pets\\
$\text{Q}_2$ & For each of those, what is the maximum age? \\
$\text{S}_2$ & SELECT max(pet\_age), pettype FROM pets GROUP BY pettype\\
$\text{Q}_3$ & What about the average age? \\
$\text{S}_3$ & SELECT avg(pet\_age), pettype FROM pets GROUP BY pettype \\
\hline %inserts single line
\end{tabular}
}
\caption{An example of \LCdSP from \Sparc~\cite{yu2019sparc}, where each SQL query $S_i$ is the LF of the question $Q_i$.}
\label{tab:CoSQL} % is used to refer this table in the text
\end{table}
